First Light And Reionization Epoch Simulations (FLARES) XXI: The UV Indices of Galaxies in the Early Universe

UV absorption line indices trace chemical enrichment and star formation histories in high-redshift galaxies, yet their reliability as quantitative stellar metallicity, Z*, diagnostics remains uncertain. In this work, we combine synthetic spectral modelling with cosmological simulations to assess the behaviour of rest-frame UV indices in the early Universe. Using the forward-modelling package Synthesizer, we compute equivalent widths for UV indices based on BPASS stellar population synthesis models and examine their sensitivity to metallicity, star formation history, nebular emission, and model assumptions. We first investigate idealised stellar populations to establish the metallicity dependence of each index. Most indices show increasing equivalent width with metallicity, although the strength and linearity of this relation varies between features. The 1719 Angstrom index exhibits one of the most stable correlations with stellar metallicity, while the 1460 Angstrom index shows stronger sensitivity to nebular emission, bursty star formation, and model-dependent effects at high metallicity. We then apply these models to galaxies from the First Light and Reionization Epoch Simulations, FLARES, which provide realistic star formation and chemical enrichment histories. The simulated galaxy populations reproduce a stellar mass-metallicity relation and allow the UV indices to be tested in composite spectra. Although scatter increases due to population mixing and stochastic enrichment, the overall metallicity trends remain largely preserved. These predictions provide a theoretical framework for interpreting rest-frame UV spectra from JWST and future surveys, supporting the use of UV absorption indices as complementary tracers of stellar metallicity in early galaxies.

==> Sections/app.tex <==
\section{Comparison of machine learning methods}\label{sec:first_appendix}

\subsection{Other methods}

We trialled two machine learning methods in addition to XGBoost -- Extremely Randomised Trees (ERT) and neural networks. For these models, our method for hyperparameter optimisation and model training was the same as that outlined in Section \ref{sec:ml.method}. To evaluate the usefulness of machine learning, we also obtained predictions for a simple model, fitted using linear least squares regression. 

\subsubsection{Extremely Randomised Trees}

Like XGBoost, Extremely Randomised Trees (ERT) is an ensemble method that combines the results of multiple CARTs. However, instead of generating trees sequentially, ERT averages the predictions of a large number of trees that have been trained independently. The split points of each tree are chosen randomly for each feature. We used the scikit-learn \cite[]{scikit-learn} implementation of ERT. The hyperparameters for each ERT model were obtained from the following hyperparameter grid: `min\_samples\_split': [10, 300, step=10], `min\_samples\_leaf': [10, 300, step=10], `n\_estimators': [10, 500, step=10].

\subsubsection{Neural Networks}

A neural network consists of layers of nodes. At each node, a mapping is performed using a specified activation function. The result of this mapping is passed to nodes in the subsequent layer, where the data is again transformed. Each connection between nodes is associated with a weight. Training a neural network involves adjusting these weights in order to reduce the loss. We used the Keras \cite[]{chollet2015keras} implementation of neural networks. For hyperparameter optimisation, we used the following grid: `neurons': [1, 30, step=1], `batch\_size': [25, 500, step=25], `epochs': [100, 1200, step=50], `n\_layers': [1, 20, step=1].

\subsubsection{Linear least squares regression}

The fitting function we use is a linear combination of the spectral diagnostics up to third order (we found that going to higher order than this leads to minimal improvement). To obtain predictions, the model was fitted using the training data, and the $R^2$ score was computed for the fitted model applied to the test data. The final $R^2$ score was averaged over a 5-fold cross-validation.

\subsection{Comparison}

We find that in general, the machine learning methods make better predictions than the fitting function we used. Of the three machine learning models, XGBoost performs marginally better for all physical properties, with the exception of stellar age. Although all three models performed similarly for the most part, the tree-based ensemble methods were quicker to optimise and train.

\begin{figure}
    \includegraphics[width=\columnwidth]{figs_LS/cubereg_ert_mlp_xgb_compare r2.png}
	\caption{$R^2$ values obtained for the three machine learning models (XGBoost, Extremely Randomised Trees, neural network). We also used linear least squares regression \label{fig:models_r2}}
\end{figure}
